Hidden Markov Models derived from Behavior Trees

Behavior trees are rapidly attracting interest in robotics and human task-related motion tracking. However no algorithms currently exist to track or identify parameters of BTs under noisy observations. We report a new relationship between BTs, augmented with statistical information, and Hidden Markov Models. Exploiting this relationship will allow application of many algorithms for HMMs (and dynamic Bayesian networks) to data acquired from BT-based systems.

==> BT-HMM-Paper/raw_theory_matl.tex <==
% Raw Theoretical BT Material 


%%%%** Section 5.1.5 
\subsubsection{  For each ABT, there is a unique HMM}\label{UniqueHMM}
\paragraph{Proof:}
        \begin{enumerate}
            \item Assume the ABT has $l$ leaves, numbered from left to right. Left to right is   the
            conventional  direction used by selector ($\to$) and sequence (?) nodes in the BT literature.
            
            \item Create a HMM state for each ABT leaf, and two additional terminal HMM states,
            $O_S$ and $O_F$, representing overall success or failure of the ABT, so that the HMM dimension is $n = l+2$.
            
            \item By definition of BT nodes, for each leaf, $j$, belonging to a specific BT, 
            there is a unique successor leaf to which the BT will transition on success, $S_s$
            which belongs to another leaf/HMM state, and another unique leaf/HMM state to which it will transition on failure, $S_f$.
            
            \item Because of the left to right structure above, if the system is in state $j$ (i.e running leaf $j$), then
            \[
            S_s > j \; \mathrm{and} \; S_f > j
            \]
            
            \item Thus the resulting HMM transition matrix, $A$  will be $n\times n$,
            upper diagonal, and each row will contain exactly 2 non zero entries ($S_s$ and $S_f$ such 
            that $A_{j,Ss} \neq 0, A_{j,Sf} \neq 0), A_{jSs}+A_{jSf}=1$ and
            $A_{jSs}=P(S)_j, A_{jSf}=1-P(S)_j$
            
            \item The HMM observation densities $B_j$ are the same as the ABT observation densities.
            
            \item We can thus construct a unique HMM for each ABT.
        \end{enumerate}

%%%%** Section 5.1.6 
\subsubsection{There is more than one BT for each HMM $A$ matrix derived above.}\label{morethan1bt}
\paragraph{Proof:}
        \begin{enumerate}
            \item Element $A_{ij}$ is defined  above as the probability of a transition from State $i$ to State $j$, however, 
            it does not contain information about whether the transition is associated by the BT
            with Success or Failure of the leaf $i$. 
            
            \item We thus will sometimes augment the HMM $A$ matrix to 
            \[
            A_{ijk} = P( i\to j |  O_{ik})
            \]
            Adding the outcome,
            \[
             O_{ik}   \in \{  0,1 \}
            \]
            where $O_{i1} = 1$ if the outcome of leaf $i$ is Success, and 
             $O_{i1} = 0$ if the outcome of leaf $i$ is Failure. 
            corresponds to the outcome of leaf/state $i$ ($O_{i2} = 1-O_{i1}$).
            Since each BT leaf has only one outcome, for each $i,j$, then either $O_1$ or $O_2$ must be 0. 
            
            \item Thus for each row in $A$, containing two non-zero probabilities which add to 1, there are two permutations, S/F and F/S,
            giving more than one BT.
            
            \item When augmented as in Step 2, there is only one BT for each HMM as constructed in \ref{UniqueHMM}.
        \end{enumerate}
        

\subsubsection{Proposition}\label{sequentialpathway}
In the state evolution of a BT, there is at least one possible pathway
(determined by S/F outcomes of the leaves) 
in which all $l$ leaves are executed in numerical order (Figure \ref{BTbasicpathway})
such that the BT visits each leaf in turn.


%%%%** Figure 5 
\begin{figure}[h]\centering
  \includegraphics[width=4.0in]{01156.png}
\caption{Any BT must have a sequential pathway for a certain set of S/F outcomes.}\label{BTbasicpathway}
\end{figure}


\paragraph{Proof:} 
\begin{enumerate}

    \item Assume all leaves must have at least one input path.  If any leaf has no input path, then it will never
    be executed and should not be in the BT.
    
    \item By convention, BT leaves are numbered from left to right.
    \item Each leaf can belong to a Selector or Sequence parent node.
    \item If leaf $j$ is not the last (rightmost) leaf of its parent then the proposition for 
    leaf $j\to j+1$ is trivial by the definition of Sequence and Selector nodes.
    \item If leaf $j$ is the last (rightmost) leaf of a Sequence or Selector, and control is passed to
    that leaf, then the parent's result is the same as the leaf's result, also by definition of Sequence and Selector nodes.
    \item For any Sequence or Selector node which is a parent of leaf $i$, at least one path coming
    out must go to a leaf $j>i$ (unless leaf $j$ is the rightmost node in the BT).    
    \item If the parent is not rightmost of the leaves belonging to its parent, then the result is trivial.
    \item If the parent IS rightmost, then by induction it will lead either to Output (the root node returns and the BT execution is over) 
    or to another higher level node as non-rightmost.
    \item Thus there must be a path from node $i$ to $i+1$.
\end{enumerate}

\subsubsection{Implication:}\label{HMMConstraints}
Considering these results, the following constraints define the set of
    HMM State-Transition-Matrices ($A$) which correspond to an Augmented BT:
    \begin{enumerate}
        \item $A$ must be upper diagonal (\ref{UniqueHMM} steps 4,5).
        \item $A$ must have exactly 2 non-zero entries per row  (\ref{UniqueHMM} steps 4,5).
        \item $A_{i,i+1} \neq 0$ (\ref{sequentialpathway}).
    \end{enumerate}


%%%%** Section 5.1.8 
\subsubsection{Reverse Mapping: HMM$\to$ BT}
With the above definition, we can investigate the reverse mapping: Given an $A$ matrix with the above constraints, what
is the corresponding BT?

First we consider how many BTs are possible for each $A$ matrix:

\subsubsection{How many BT's are possible for $l$ BT leaves?}
    \begin{enumerate}
    
        \item Since there is a unique HMM for each BT, we can answer the equivalent question: ``How many HMMs of $l+2$ states meet the constraints of \ref{HMMConstraints}?"
    
        \item Each element just above the diagonal,  $A_{i,i+1}$, must be non-zero because every BT has a sequential pathway. But further, the
        probability in  $A_{i,i+1}$ may represent Success (if leaf $j$ belongs to a Sequence Node) or Failure (if leaf $j$ belongs to a Selector
        Node).  However, the last leaf, leaf $l$, must transition to Os on Success (and to Of on Failure), so there are $2^{l-1}$ permutations of S/F outcomes
        for leaves $i=1..l$ (Fig. \ref{AmatrixFig}).

%%%%** Figure 6 
\begin{figure}[h]\centering
\includegraphics[width=2.0in]{01157.png}
\caption{Constraints on $A$ matrix of HMM derived from BT.}\label{AmatrixFig}
\end{figure}
        \item There must be 2 non-zero entries per row.
        At this step we ignore their Success/Failure status which were taken into account in steps 1 and 2.
        
        \item For row 1, there are $l+2$ columns, but the $A_{1,1}$ element must be zero, and we have already taken into account the 
        $A_{1,2}$ element.   Thus there are thus $l+2-2 = l$ available columns, only 1 of which can be non-zero.
        \item For row $i$, there are $l+2-(i+1) = l+1-i$ columns from which to
        independently choose.
        \item Thus there are
        \[
        \Pi (l,l-1, \dots 2, 1) = l!
        \]
        permutations of the second non-zero elements in   rows $1 \dots l$.
        \item Combining, the total number, $m_{BT}$, of BTs for an $l\times l$ $A$ matrix (augmented with the $O_S, O_F$ rows and columns) would
        be
        \[
        m_{BT} = 2^{l-1}l!
        \]

        \end{enumerate}
 
 For 10 leaf nodes there are about 186 billion possible behavior trees. 

